A cost of capital approach to determining the LGD discount rate

Loss Given Default (LGD) is a key risk parameter in determining a bank's regulatory capital. During LGD-estimation, realised recovery cash flows are to be discounted at an appropriate rate. Regulatory guidance mandates that this rate should allow for the time value of money, as well as include a risk premium that reflects the "undiversifiable risk" within these recoveries. Having extensively reviewed earlier methods of determining this rate, we propose a new approach that is inspired by the cost of capital approach from the Solvency II regulatory regime. Our method involves estimating a market-consistent price for a portfolio of defaulted loans, from which an associated discount rate may be inferred. We apply this method to mortgage and personal loans data from a large South African bank. The results reveal the main drivers of the discount rate to be the mean and variance of these recoveries, as well as the bank's cost of capital in excess of the risk-free rate. Our method therefore produces a discount rate that reflects both the undiversifiable risk of recovery recoveries and the time value of money, thereby satisfying regulatory requirements. This work can subsequently enhance the LGD-component within the modelling of both regulatory and economic capital.

==> MeetingNotes.tex <==
--- General To-do
    - Reposition background of Solvency II into sec. 2
    - Expand on Witzany2009 in sec 2, criticise all faults, and show how our work differs


2023-Feb-03 (Intro meeting):
- Focus on retail data? Workout LGD therefore?

2023-Feb-10:
-Removed AB's FirstRand-affiliation
-To-Do:
    - read section 3 (solvency), 3.1 (regulatory/economic capital for recovery risk)
    - study Tasche2004, given its proximity to current study
    - Refine intro & section 2.2

2023-02-24: To-do | Everyone
    - Consider summarising section 2.1 and repositioning to introduction
    - move parts of section 3 and 3.1 into "background" section 2, so that the remainder of section 3 is actually "method-focused"
    - Section 4: Refine graphs, 1: overall density; 2: how did density change over time.

2023-03-10: Milestones | AB
    - Refined introduction and reordered ideas, focusing on first explaining (succinctly) the collection process and its affect on L. This description leads to the first diagram, illustrating the two main outcomes of resolving a default

2023-03-10: To-Do | AB
    - Intro: Refine discount rate as main thrust of paper
    - Intro: Refine foreshadowing of paper's main contribution ("cost of capital" approach)

2023-03-17: Milestones | AB
    - Embedded VanGestel2009 (book) regarding LGD, in particular, discount rates.
    - Refocused par. 3 by removing discussion on all LGD-methods, instead focusing only on workout method (greater relevance to our paper)
    - Finessed Fig. 2 (workout method)
    - Moved E[L] and V[L] from Intro to sec 3.2
    - Excavated regulatory principles on discount rates (Basel2005) from sec. 2 to Intro, since limited prescription forms part of the "problem"
    - Refined "Solution"-part of intro (CoC-approach)

2023-07-03: Renewed To-Do | AB
    - Refine section 2 (background)
    - study Tasche2004, given its proximity to current study
    - study Witzany2009, given its proximity to current study
    - Read & review rest

2023-07-14: Milestones | AB
    - Sec. 1: par. 4: removed sentence about "illogical LGD-values"
    - Sec. 3: Restructured Solvency II subsection and Basel subsection together and moved as part of "background". Section 3 is now purely method, with finessed section titles
    - Sec. 2.0 par. 1: refinement in-progress
    - Sec. 3 par. 1: refinement in-progress
    - General questions:
        - Article format still Orion, given we intend to submit to ASSA?
            - Needs follow-up from Conrad
        - sec. 1: link to codebase?
            - We don't want to, this is not a "model" per se
        - sec. 2.2: Vasicek?
        - Missing write-offs histogram in fig 3?
            - Can re-embed
            - Can remove kernel density estimates
    - Questions: method:
        - care about $C_t$ definition?
        - distribution of $X_t$ and/or $t$?
        - clarify process for finding $\delta$ in Eq. 8


2023-07-17: Milestones | AB
    - Sec. 1 par. 3: Transformed $\tau_d$ and $\tau_r$ to be functions of account i (or relationship path i), in line with Scheule2020, which I quite like. Though kept $u$ without $i$ to simplify notation.
        - Tried to apply in section 3 regarding $\tau_r(i)$ and $\tau_d(i)$, though discovered new question
    - Sec. 1 par. 3: Simplified Eq. 1


2025-02-xx: Notes | AB
    - Finessed abstract
    - Inserted NITheCS affiliation
    - Refined introduction and signpost-paragraph
    - Crafted Witzany2009 summary
    - Finalized "earlier methods" literature study
    - Refined Solvency II section
    - Questions: 
        - Do we want "$\mathrm{m}$" for all instances where the subscript does not constitute an index of sorts? Only asking since I thought it prudent to change the $\rho$-variants to normal Roman (instead of italics).
